3D generation on ImageNet

Existing 3D-from-2D generators are typically designed for well-curated single-category datasets, where all the objects have (approximately) the same scale, 3D location, and orientation, and the camera always points to the center of the scene. This makes them inapplicable to diverse, in-the-wild datasets of non-alignable scenes rendered from arbitrary camera poses. In this work, we develop a 3D generator with Generic Priors (3DGP): a 3D synthesis framework with more general assumptions about the training data, and show that it scales to very challenging datasets, like ImageNet. Our model is based on three new ideas. First, we incorporate an inaccurate off-the-shelf depth estimator into 3D GAN training via a special depth adaptation module to handle the imprecision. Then, we create a flexible camera model and a regularization strategy for it to learn its distribution parameters during training. Finally, we extend the recent ideas of transferring knowledge from pre-trained classifiers into GANs for patch-wise trained models by employing a simple distillation-based technique on top of the discriminator. It achieves more stable training than the existing methods and speeds up the convergence by at least 40%. We explore our model on four datasets: SDIP Dogs 256x256, SDIP Elephants 256x256, LSUN Horses 256x256, and ImageNet 256x256, and demonstrate that 3DGP outperforms the recent state-of-the-art in terms of both texture and geometry quality. Code and visualizations: https://snap-research.github.io/3dgp.

==> figures/architecture-details.tex <==
\begin{figure}
\topspace
\centering
\includegraphics[width=\textwidth]{images/architecture-details.pdf}
\caption{Left: camera generator architecture. Right: depth adaptor architecture.}
\label{fig:architecture-details}
\botspace
\end{figure}

==> figures/camera-distribution.tex <==
\begin{figure}
\topspace
\centering
\includegraphics[width=\textwidth]{images/camera-distribution.pdf}
\caption{Comparing different regularization strategies for camera generator $\C$.}
\label{fig:camera-distribution}
\botspace
\end{figure}


==> figures/epigraf.tex <==
\begin{figure}
\topspace
\centering
\includegraphics[width=\textwidth]{images/epigraf-architecture.pdf}
\caption{EpiGRAF (left) is purely NeRF-based and uses the tri-plane backbone~\cite{EG3D} with the StyleGAN2~\cite{StyleGAN2} decoder (but without the 2D upsampler). Our discriminator (right) is also based on StyleGAN2, but is modulated by the patch location and scale parameters. We use the patch-wise optimization for training~\cite{GRAF} with our proposed Beta scale sampling, which allows our model to converge $\times$2-3 faster than the upsampler-based architectures despite the generator modeling geometry in full resolution (see Tab~\ref{tab:main-results}). The image is copied from the original paper with the permission of their authors.}
\label{fig:architecture}
\botspace
\end{figure}



==> figures/leres-data.tex <==
\begin{figure}
\topspace
\centering
\includegraphics[width=\textwidth]{images/epigraf-architecture.pdf}
\caption{EpiGRAF (left) is purely NeRF-based and uses the tri-plane backbone~\cite{EG3D} with the StyleGAN2~\cite{StyleGAN2} decoder (but without the 2D upsampler). Our discriminator (right) is also based on StyleGAN2, but is modulated by the patch location and scale parameters. We use the patch-wise optimization for training~\cite{GRAF} with our proposed Beta scale sampling, which allows our model to converge $\times$2-3 faster than the upsampler-based architectures despite the generator modeling geometry in full resolution (see Tab~\ref{tab:main-results}). The image is copied from the original paper with the permission of their authors.}
\label{fig:architecture}
\botspace
\end{figure}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/acknowledgments.tex <==
\subsubsection*{Acknowledgments}

We thank Willi Menapace, Rameen Abdal, Menglei, Ceyuan Yang and Min Jin Chong for the helpful discussions.
We thank Ahmed Abdelreheem for ...
We thank Snap and KAUST Ibex team for maintaining the compute infrastructure.


==> sections/method_old.tex <==
\section{Our model}\label{sec:method}

\input{figures/architecture-overview}
\input{figures/camera-parametrization}

\subsection{Backbone}\label{sec:method:backbone}
We use EpiGRAF~\citep{EpiGRAF} as our generator backbone due to its fast training speed and reasonable generation quality. It is a GAN-based 3D generator which does not use a 2D upsampler and instead utilizes tri-planes~\citep{EG3D, TensoRF} with multi-scale patch-wise training~\citep{GRAF, AnyResGAN}.

First, mapping network $\M(\bm z, \bm c)$, represented as a 2-layer MLP, takes random noise $\bm z \sim \Nstd \in \R^{512}$ and 
random class label $\bm c \sim U\{0, 1, ..., N_\text{cls}\} \in \N$
and produces latent code $\bm w \in \R^{512}$.
Then, synthesis network $\Ss(\bm w)$, parametrized as a StyleGAN2-based~\citep{StyleGAN2-ADA} convolutional decoder, uses this latent code $\bm w$ and outputs tri-plane features $\bm T = (\bm T^{xy}, \bm T^{yz}, \bm T^{xz}) \in \R^{3 \times 512 \times 512 \times 32}$.
Tri-planes are a compressed representation of a voxel feature grid, where feature vector $\bm t_{xyz} \in \R^{32}$ in coordinate $(x, y, z) \in \R^3$ is calculated by projecting the coordinate on the planes, bi-linearly interpolating the nearby features and averaging the features from the planes.
To obtain the color and density in coordinate $(x,y,z)$, one passes the corresponding feature $\bm t_{xyz}$ through a tri-plane decoder $\Fd(\bm t_{xyz}) = (\text{RGB}, \sigma) \in \R^4$, parametrized as a lightweight 2-layer MLP, and obtains the color $\text{RGB} \in \R^3$ and density $\sigma \in \R_+$.
Finally, volumetric rendering~\citep{NeRF} is performed on top of the tri-planes, using a random camera pose $\bm\phi = (\bm\phi_\text{ext}, \bm\phi_\text{int}) \in \R^{25}$ (consisting on extrinsic $\bm\phi_\text{ext} \in \R^{4 \times 4}$ and intrinsic $\bm\phi_\text{int} \in \R^{3 \times 3}$ camera parameters), and random patch parameters $\bm\psi = (s, \delta_x, \delta_y) \in \R^3$ (consisting on patch scale $s \in [0, 1]$ and horizontal/vertical patch offsets $\delta_x, \delta_y \in \R$).
EpiGRAF renders only $64^2$ pixels on each iteration instead of the full resolution $256^2$, which significantly improves its training speed.
Its discriminator closely follows the architecture of StyleGAN2's discriminator~\citep{StyleGAN2-ADA} and conditions it on patch parameters using projection discriminator~\citep{ProjectionDiscriminator} and hypernetwork-based~\citep{Hypernetworks} strategies.
It is trained with the traditional adversarial loss with $\Rpenalty$ gradient penalty~\cite{R1_reg}:

\begin{equation}
\Ladv = \expect[\bm x, \bm c, \bm \phi]{-\log \D(\G(\bm z, \bm c, \bm\phi), \bm c)} + ... + \Rpenalty
\end{equation}

\todo{should we put in related work?}

\subsection{Model overview}\label{sec:method:overview}
We develop three techniques on top of EpiGRAF to make it work on non-alignable datasets.
First, we relax its camera model and learn the distribution over its position, field-of-view and look-at.
The distribution over field-of-view and look-at is conditioned on the scene noise code $\bm z$ to make $\G$ capable to zoom into the suitable regions of the scene.
This allows to model datasets, which have non-alignable objects in different positions and zooms, or which might have multiple objects on the same scene.
Second, we build a technique to utilize an off-the-shelf imperfect monocular depth estimator to incorporate the 3D bias into the generator.
Currently, 3D generators trained on real data use two ways to incorporate a 3D bias: 1) dataset alignment; and 2) ground-truth camera poses for real images.
None of these sources is applicable for in-the-wild data, which raises a need of another way.
We estimate the depth maps for real images and pass them as the 4-th channel to $\D$.
For fake samples, we render the depth map from the synthesized radiance field, adapt them with a shallow depth adaptor to account for imperfections in the depth estimator, and also pass as the 4-th channel to $\D$.
This gives geometric supervision through adversarial training.
Moreover, some images might contain even several objects, that is why it is necessary for $\G$ to learn this distribution
Finally, 

\subsection{Adversarial depth supervision}\label{sec:depth-adaptor}
Depth estimator is the most important component of our system.
In the original paper, EpiGRAF was trained on two types of datasets: frontal-view real datasets with known camera positions and multi-view 360$^\circ$ synthetic datasets, with all of them being aligned.
This gives strong 3D inductive bias to the model, which is not accessible for in-the-wild data: it has typically frontal views of non-alignable scenes which we do not know even the camera parameters for.
To instill the 3D bias into the model, we develop a strategy of using imperfect estimated depth maps.
Its key advantage is that it is very generic and readily applicable for many object categories.

The main idea is concatenating the depth map as a 4-th channel to the discriminator RGB input.
For real images, we take their depth maps, estimated with LeReS monocular depth estimator~\citep{LeReS}\footnote{\leresrepohref}.
It produces depth maps in the range $[0, 2^{16}]$, which we normalize into the [-1, 1] range.

Producing depth maps as fake images is more complicated.
First, we render raw depths $\tilde{\bm d}$ from NeRF via volumetric rendering:
\begin{align}
\bm d = \int_{t_n}^{t_f} T(t) \sigma (\bm r(t)) t dt,
\end{align}
where $t_n, t_f \in \R$ are near/far planes (we always use $t_n = 0.75$ and $t_f = 1.25$).
It is then shifted and scaled from its $[n, f]$ range into $[-1, 1]$:
\begin{align}
\bar{\bm d} = 2 \cdot \frac{\bm d - (t_n + t_f + b) / 2}{t_f - t_n - b}
\end{align}
where $b \in [0, (t_n + t_f) / 2]$ is an additional learnable shift needed to account for the empty space in front of the camera which does not appear for the estimated depth maps from the monocular depth estimator.
We cannot feed those depth maps to $\D$ as they are, because it will force $\G$ to learn all the prediction artifacts from $\E$.
That's why $\bar{\bm d}$ is fed to the depth adaptor $\A$ to produce an adapted depth map $\bm d_a = \A(\bm d) \in \R^{256 \times 256}$.
This depth $\bm d_a$ is then concatenated as the 4-th channel to the input and passed to $\D$.

This happens because the depth estimator is not perfect: 1) it produces noisy artifacts; 2) ignores high-frequency details; and 3) simply makes prediction mistakes.
One could try running the depth estimator on top of predicted images, but this is undesirable, since 1) it is computationally heavy; and 2) $\G$ is trained patch-wise and does not make good predictions for just patches.
Moreover, in our experiments we noticed that it is easy for $\G$ to fake depth and it could learn to spoof the depth estimator.
That is why we define a depth adaptor $\A$ which takes a rendered depth $\bm d$ and adapts it into $\bm d_a = \A(\bar{\bm d})$.
We depict its architecture in Fig~\ref{fig:depth-adaptor}.

We want to constraint $\bm d_a$ to deviate as little as possible from $\bar{\bm d}$.

We want the adapted depth map $\bm d_a$ to be a small adjustment over the original one $\bm d$, since it is the original depth map.
An intuitive attempt to enforce this would be 
Depth adaptor $\A$ is a 3-layer convolutional network which takes the rendered depth map $\bm d$ and predicts its adjustments:
\begin{equation}
\A(\bm d) = [\bm d_a^{(1)}, \bm d_a^{(2)}, \bm d_a^{(3)}, , \bm d_a^{(\ell)}]
\end{equation}
We want each depth map $\bm d_a^{(\ell)}$ to be a small adjustment over the previous one $\bm d_a^{(\ell - 1)}$ so that the geometry from .
We compare to the normal prediction strategy and show that it is better to do things like we do.

\input{figures/depth-adaptor}

\subsection{Learnable ``ball-in-sphere'' camera distribution}\label{sec:method:camera}
Current 3D generators parameterize the camera distribution the following way.
Its position is sampled on a fixed-radius sphere with fixed hand-crafted intrinsic parameters and its look-at position is always the $(0, 0, 0)$ coordinate.
Such a parametrization assumes that all the objects are centered, equally rotated and zoomed with respect to some canonical alignment.
However, 3D scenes in the-wild-data are inherently non-alignable: it is impossible to find a common canonical for e.g., a mountain landscape and a bunch of kittens.
To relax those assumptions, we introduce our camera parametrization.
While it works when all the objects are aligned, it is not suitable for in-the-wild data.

Moreover, when trained on a single category, our generator learns implicit alignment of the objects.



To the best of our knowledge, CAMPARI~\citep{CAMPARI} is the only work which also learns the camera distribution.
They 


\subsection{Knowledge distillation for Discriminator}\label{sec:method:distillation}
Recent works have demonstrated from employing pretrained off-the-shelf models to improve the convergence of GANs~\cite{ProjectedGANs, EnsemblingOffTheShelfModels, StyleGAN-XL, InstanceConditionedGAN}.

The most popular strategy is developed in StyleGAN-XL~\cite{StyleGAN-XL}, which achieves.
These techniques work by using an off-the-shelf model as a discriminator while freezing most of the weights.
The problem to benefit from them in our scenario is that 

\subsection{\metricfullname}
The main geometry failure case of tri-plane (and MPI ~\cite{GMPI})-based 3D generators is the flatness of the objects, when the frontal feature plane takes all the load in generating the content~\citep{EG3D, EpiGRAF, GMPI, IDE-3D}.
To detect and measure this failure case in such generators, we propose \metricfullname (\metricname), which is computed the following way.
Compute 256 depth maps for the frontal view, while cutting the 50\% lowest density to 0.0 (this is needed to remove spurious density).
Then normalize the depth maps with near and far plane (for EG3D, we use its average ones --- see Appx~\ref{ap:metric-details}).
Then we split into 64 bins, compute histograms (for each density map independently).
Then we treat those values inside each histogram as probabilityies, compute entropy, then exponentiate and average.
\begin{align}
\text{Non-Flatness Score} = \frac{1}{N}\sum_{i=1}^N\exp\left[ -\frac{1}{h \cdot w} \sum_{j=1}^B b(\bm d^{(i)})_j \right],
\end{align}
where $b(\bm d^{(i)})_j$ --- the number of values in the $j$-th bin of the $i$-th depth map $\bm d^{(i)}$, $N$ is the number of samples we use (we always use 256), $B$ is the number of bins (we always use 64).

We provide intuition on it in Fig~\ref{fig:metric-vis}.


As noted in Sec.~\ref{sec:limitations}, \metricname is not able to detect the quality of the geometry, but is a useful metric to detect and measure flatness of the generations, which is the most popular failure case of tri-plane-based generators.
We provide the details on this metric in Appx~\apref{ap:metric-details}.


\subsection{Training}
For ImageNet experiments, we double the number of channels in EpiGRAF, both in $\Ss$ and $\D$.
We train all the models with Adam optimizer~\cite{Adam} with the learning rate of 0.002 and $\beta_1 = 0.0, \beta_2 = 0.99$ with the non-saturating loss.
We also decrease $\Rpenalty$ weight $\gamma$ to 0.01 to give more flexibility to $\D$: we noticed that using our knowledge distillation scheme allows to reduce it without leading to a collapse, like in BigGAN~\cite{BigGAN}.
For LSUN Cats $256^2$ we use $\gamma=0.1$ since it is less diverse dataset than ImageNet.
Following EpiGRAF, we train the model patch-wise with $64^2$-resolution patches and use their proposed $\beta$ scale sampling strategy without any modifications.
For additional details, see Appx~\ref{ap:implementation-details}.

The overall use which we use during training consists on:
\begin{equation}
123
% \Ltotal(\bm\theta_\G, \bm\theta_\C, \bm\theta_\C, \bm\theta_\D) = \Ladv(\bm\theta_\G, \bm\theta_\C, \bm\theta_\C, \bm\theta_\D) + \Lkd(\bm\theta)
\end{equation}


==> tables/geometry-old.tex <==
\begin{table*}[t]
\caption{The influence of Depth Adaptor ($\A$) and Knowledge Distillation (KD) on visual quality (FID) and geometry (NFS). KD provide a significant boost in terms of visual quality, however does not affect the geometry. $\A$ on the other hand significantly improves geometry. For completeness we also provide 2D baseline StyleGAN2 (with KD) in the last row. In the last column we compare the training cost of different medods. \green{From this table it seem that the best is $\depthprob = 0.5$, also what is ADS maybe it simplier to write +$\A$?}}
\label{tab:2d-experiments}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{SDIP Dogs$_\text{40k}$} & \multicolumn{2}{c}{SDIP Elephants$_\text{40k}$} & \multicolumn{2}{c}{LSUN Horses$_\text{40k}$} & Training cost \\
& FID$_\text{2k}$ $\downarrow$ & \metricname $\uparrow$ & FID$_\text{2k}$ $\downarrow$ & \metricname $\uparrow$ & FID$_\text{2k}$ $\downarrow$ & \metricname $\uparrow$ & (A100 days) \\
\midrule
EG3D & 26.0 & 12.3 & 10.7 & 2.85 & 5.43 & 15.3 & 3.7  \\
~+ wide camera & yy.y & yy.y & yy.y & yy.y & yy.y & yy.y & 3.7  \\
EpiGRAF & 25.6 & 3.53 & 8.24 & 12.9 & 6.45 & 9.73 & 2.3 \\ 
3DGP \ours & yy.y & yy.y & yy.y & yy.y & yy.y & yy.y & yy.y \\ 
\midrule

\midrule
3DGP w/o ADS, w/o $\C$ & 8.59 & 1.42 & 7.46 & 9.52 & 3.29 & 8.04 & 2.3 \\
~+ ADS, $\depthprob = 0.0$ & 8.13 & 3.14 & yy.y & yy.y & 3.41 & 1.24 & 2.6 \\
% ~+ ADS, $\depthprob = 0.0$, $N_\ell=1$ & 10.7 & 29.8 & xx.x & xx.x & 6.11 & 28.63 & 2.4 \\
% ~+ ADS, $\depthprob = 0.1$ & 8.72 & 6.27 & 6.02 & 17.46 & 3.66 & 1.44 & 2.6 \\
~+ ADS, $\depthprob = 0.25$ & 9.57 & 33.21 & 6.26 & 33.45 & 4.33 & 32.68 & 2.6 \\
~+ ADS, $\depthprob = 0.5$ & 9.25 & 36.9 & 7.60 & 30.69 & 5.27 & 32.24 & 2.6 \\
~+ ADS, $\depthprob = 1.0$ & 12.2 & 27.2 & 12.1 & 26.0 & 8.24 & 27.7 & 2.5 \\
% ~+ ADS, $\depthprob = 0.25 \rightarrow 0.1$ & 8.88 & 32.06 & 6.81 & 30.67 & 4.15 & 26.43 & 2.6 \\
\midrule
StyleGAN2 (with KD) & 6.24 & 0.0 & 3.94 & 0.0 & 2.57 & 0.0 & 1.5 \\
\bottomrule
\end{tabular}
}
\end{table*}

